Uncoordinated Access to Serverless Computing in MEC Systems for IoT

Edge computing is a promising solution to enable low-latency IoT applications, by shifting computation from remote data centers to local devices, less powerful but closer to the end user devices. However, this creates the challenge on how to best assign clients to edge nodes offering compute capabilities. So far, two antithetical architectures are proposed: centralized resource orchestration or distributed overlay. In this work we explore a third way, called uncoordinated access, which consists in letting every device exploring multiple opportunities, to opportunistically embrace the heterogeneity of network and load conditions towards diverse edge nodes. In particular, our contribution is intended for emerging serverless IoT applications, which do not have a state on the edge nodes executing tasks. We model the proposed system as a set of M/M/1 queues and show that it achieves a smaller jitter delay than single edge node allocation. Furthermore, we compare uncoordinated access with state-of-the-art centralized and distributed alternatives in testbed experiments under more realistic conditions. Based on the results, our proposed approach, which requires a tiny fraction of the complexity of the alternatives in both the device and network components, is very effective in using the network resources, while incurring only a small penalty in terms of increased compute load and high percentiles of delay.

==> watermark.tex <==
\usepackage{fancyhdr}
\setlength{\headheight}{15pt}

\pagestyle{fancyplain}
\fancyhf{}
\lhead{ UNPUBLISHED WORK SUBMITTED FOR PUBLICATION }
\rhead{ \fancyplain{}{\thepage} }

\usepackage{draftwatermark}

\SetWatermarkText{{\bf UNPUBLISHED WORK SUBMITTED FOR PUBLICATION}}
\SetWatermarkLightness{0.8}
\SetWatermarkScale{0.8}

